Analysis of Feature Representations for Anomalous Sound Detection

In this work, we thoroughly evaluate the efficacy of pretrained neural networks as feature extractors for anomalous sound detection. In doing so, we leverage the knowledge that is contained in these neural networks to extract semantically rich features (representations) that serve as input to a Gaussian Mixture Model which is used as a density estimator to model normality. We compare feature extractors that were trained on data from various domains, namely: images, environmental sounds and music. Our approach is evaluated on recordings from factory machinery such as valves, pumps, sliders and fans. All of the evaluated representations outperform the autoencoder baseline with music based representations yielding the best performance in most cases. These results challenge the common assumption that closely matching the domain of the feature extractor and the downstream task results in better downstream task performance.

==> sections/old/approach.tex <==
\section{Approach}
\label{sec:approach}
We assume that the ASD system monitors the entity for an application specific, predefined period of time (decision horizon) until the degree of abnormality needs to be estimated.
Thus, the space of all normal and anomalous operation Mel-spectrograms is given by (\ref{eq:D}) and (\ref{eq:Dbar}), respectively.
\begin{equation}
    \label{eq:D}
    \mathcal{D}=\{M \in \mathbb{R}^{\hat{F} \times T}\,\, \vert \,\, \texttt{label}(M) = 0\}
\end{equation}
\begin{equation}
    \label{eq:Dbar}
    \Bar{\mathcal{D}}=\{M \in \mathbb{R}^{\hat{F} \times T}\,\, \vert \,\, \texttt{label}(M) = 1\}
\end{equation}
where $\texttt{label}: \mathbb{R}^{\hat{F} \times T} \rightarrow \{0,1\}$ is a labeling function that returns $0$ for a normal operation Mel-spectrogram and $1$ otherwise.
$\hat{F}$ is the number of Mel-bins and $T$ number of time frames. Note that $T$ depends on the decision horizon and the parameters used to generate the Mel-spectrogram.
The goal is to find a function $\mathcal{F}_{\Theta}$ parameterized with $\Theta$ such that
\begin{equation}
    \label{eq:goal}
    \forall(m, \Bar{m}) \in \mathcal{D} \times \Bar{\mathcal{D}}: \,\, \mathcal{F}_{\Theta}(m) < \mathcal{F}_{\Theta}(\Bar{m})
\end{equation}
In ASD, we only have access to $\mathcal{D}_{\text{train}}$ where
\begin{equation}
    \mathcal{D}_{\text{train}} \subset \mathcal{D}
\end{equation}
and the labeling function is unknown. Note that Equation~\ref{eq:goal} represents the idealized setting.\\
It is common to subdivide the computation of the final anomaly score $\mathcal{F}(X)$ into a sequence of smaller predictions that operate on a smaller timescale. For example, the decision horizon might be $10$ seconds but the ASD system outputs an anomaly score every $0.5$ seconds. This is a simple strategy to avoid overlooking subtle short-term anomalies and causes a trade-of between local and global structure. 
A score for the whole decision horizon is obtained by aggregation. In our case, we transform each Mel-spectrogram $X \in \mathcal{D}_{train}$ into a sequence of feature representations $X'\in \mathbb{R}^{D \times T'}$ by using a sliding window across the columns (time dimension). For each window of $n$ frames, a feature extractor $f: \mathbb{R}^{\Hat{F} \times n} \rightarrow \mathbb{R}^{D}$ extracts a $D$ dimensional feature vector that is more semantically compact than raw spectrogram features. Then the window is moved $h$ frames to the right.
The number of feature vectors $T'$ is given by $\frac{T-n}{h}$. Note that if $\frac{T-n}{h} \not\in \mathbb{N}$ an appropriate padding strategy has to be applied. Since no labels are available we propose to fit a gaussian mixture model (GMM) with $k$ components to the extracted features.\\
The GMM was chosen as anomaly detector as it was shown~\cite{Muller2020} to outperform other models on the task of anomalous sound detection when using features based on image transfer learning. Moreover, GMMs are fast and easy to train due to the ready availability of reliable implementations and have a sound probabilistic interpretation.\\
The anomaly score for a single feature vector $x \in \mathbb{R}^D$ is then computed by the weighted negative log-likelihood.
\begin{equation}
    \label{eq:gmm}
    \mathcal{L}(x) = -\log \sum_{i=1}^{k} \lambda_i * N(x;\mu_i, \Sigma_i)
\end{equation}
where $\mu_i$, $\Sigma_i$ and $\lambda_i$ are the mean, covariance matrix and weight of the $k$th mixture component.
Consequently, the anomaly score $\mathcal{A}$ for $X'$ is given by:
\begin{equation}
    \label{eq:Anomaly}
    \mathcal{A}(X) = \sum_{i=1}^{T'} \mathcal{L}(X_{*, i})
\end{equation}
We want to emphasize that Equation~\ref{eq:Anomaly} is highly dependent on expressive features that enable learning a meaningful notion of normality. In this work, $f$ comes in the form of a CNN that extracts a feature vector for a small patch ($\approx 1$s) of the Mel-spectrogram.\\

Let $x \in \mathbb{R}^d$ be a random variable of possible feature representations. We aim to find a probability density function (PDF) $p_X$ 
the sample space of all possible feature vectors and $P_X(x)$ a probability density function. Consequently, the event of $X$ not being normal $\bar{X}$ is given by $P(\bar{X}) = 1 - P(X)$.
\begin{equation}
    \label{eq:gmm}
    P_X(x) = \sum_{k=1}^{K} \lambda_i * N(x|\mu_i, \Sigma_i)
\end{equation}
where $\sum_{k=1}^{K}\lambda_i = 1$
% or is S simply \mathbb{R}^d ??
$$
p_{X_1,\dots X_n}(x_1, \dots x_n) = \prod_{i=1}^{n} p_X(x_i)
$$
GMM has the capability to model arbitrary densities

==> sections/old/approach_old.tex <==
\section{\uppercase{Proposed Approach}}
\label{sec:approach}
ABCDEFGH

\begin{equation}\label{eq:encoder}
   E(x) = f_n \circ f_{n-1} \circ \ldots  f_1(x)
\end{equation}

\begin{equation}\label{eq:decoder}
   D(z) = f_1^{-1} \circ f_{n-1}^{-1} \circ \ldots  f_n^{-1}(z)
\end{equation}

\begin{equation}\label{eq:ae}
   \text{AE}(x) = D \circ E(x)
\end{equation}

\begin{equation}\label{eq:mse}
   \hat{x} = \lVert x - \text{AE}(x)\rVert^2_{2}
\end{equation}

\begin{equation}\label{eq:quantile}
    \text{todo quantile loss}
\end{equation}

\begin{equation}\label{eq:gmm}
    L_{\texttt{GMM}}(x) = -\log \sum_{i=1}^{k} \lambda_i * \mathcal{N}(x;\mu_i, \sigma_i)
\end{equation}


\begin{figure}
  \centering
  \includegraphics[width=1.\linewidth]{imgs/example}
  \caption{Mel-spectrogram of normal operation sounds from a fan with background noise from a factory. An auto-encoder fails to reliably reconstruct the noisy regions. This in turn leads to high a reconstruction error on normal data, thereby obfuscating real anomalies.}
  \label{fig:example}
\end{figure}



==> sections/old/experiments_old.tex <==
\section{\uppercase{Experiments}}
\label{sec:experiments}
It has previously been demonstrated~\cite{Purohit2019} that anomalous sound detection based on simple (dense) auto-encoders yields good results for stationary sounds. Building upon this finding, our approach is specifically designed to improve results on stationary machine sounds compared to an off-the-shelf auto-encoder. In contrast, non-stationary sounds emitted from machines such as sliders and valves, were shown~\cite{Suefusa2020} to require other neural network architectures due to the difficulty of predicting the edge frames.\\
To study the efficacy of our method, we use the recently published MIMII dataset~\cite{Purohit2019}. It consists of recordings from four diffenrent machine types under normal and abnormal operation. As previously mentioned, we focus on stationary machine sounds and therefore only consider sounds from fans and pumps. Additionally, for each machine type there are sounds from four different machine models (ID $0,2,4$ and $6$). Lastly, there three exist versions of each recording where real-world background-noises from a factory are mixed with the machine sound according to a signal-to-noise ratio of $6$dB, $0$dB and $-6$dB. 
A practically applicable
and reliable anomalous sound detection system should be able to yield good results across all combinations. \\
Moreover, we closely follow the evaluation setup from~\cite{Purohit2019}. For each $10$s long recording, the corresponding Mel-spectrogram was computed with $64$ mel bands, a Hanning-window of $1024$ and a hop length of $512$. All recordings are sampled at $16$kHz and have a $16$bit bit-depth. Then we normalized the the Mel-spectrograms  $\in \mathbb{R}^{64 \times 313}$  to lie in the range $[0,1] $ and  extracted small $64 \times 5$ patches in a sliding window fashion across the time dimension (columns) with a hop length of $3$. Subsequently, the patches were flattened to yield feature vectors $\in \mathbb{R}^{320}$. Note that the columns were padded such that no column of the original Mel-spectrogram had to be discarded due to the sliding window approach. The following models were trained on every combination of machine type, machine id and signal-to-noise ratio:\\
\begin{itemize}
    \item \textbf{Dense Auto-Encoder} (AE)\\
    We usse an auto-encoder with the following architecture:\\ \texttt{Linear(320, 64, LReLU), Linear(64, 32, LReLU), Linear(32, 16, LReLU), Linear(16, 32, LReLU), Linear(32, 64, LReLU),  Linear(64, 320, $\cdot$)} where \texttt{LReLU} is the Leaky-ReLU activation function~\cite{Xu2015} with $\alpha=0.2$. The (mean squared) reconstruction error serves as anomaly score.
    \item \textbf{One-LAMP}\\
    Here the AE's$ 16$-dimensional bottleneck is used to train a GMM with $42$ mixture components with diagonal covariance matrices.
    \item \textbf{LAMP}\\
    The concatenation of all of the encoders activations is used to to train a GMM with the parameters as above. The resulting representations are $112$ dimensional.
    \item \textbf{Q-LAMP}\\
    Instead of only predicting the mean via the mean-squared error, we add two additional decoder heads to predict the $0.1, 0.5$ and $0.9$ quantile using Eq.\ref{eq:quantile}. The rest follows the LAMP framework.
    \item \textbf{Random Network Distillation} (RND)\\
    A trainable encoder is used to regress the features from another fixed and randomly initialized encoder. RND was originally proposed to improve exploration in reinforcement-learning~\cite{Burda2018}. An Ensemble of RNDs was recently used for uncertainty quantification~\cite{Ciosek2019}. The (mean squared) prediction error serves as anomaly score.
\end{itemize}

Anomalous recordings (damaged machines) were only considered at test time. We randomly set aside the same amount of normal operation recordings as there are anomalous recordings and trained the models five times across five different seeds.
During test time the same sliding-window was applied to each $10$s long recording. The segment-level anomaly scores were averaged (mean-pooling) to obtain a single score for each recording. Performance is measured in terms of the \textit{Area Under the Receiver Operating Characteristics} (AUC) which yields a complete sensitivity/specificity report.\\
The results are summarized in Table \ref{tab:results} and Table \ref{tab:results2} Each cell represents the mean AUC $\pm$ one standard deviation. Table \ref{tab:results} compares LAMP with its direct competitors while Table \ref{tab:results2} contrasts different variations of LAMP. For clarity, both tables include the results for LAMP.
\input{tables/results}


==> sections/preliminaries.tex <==
\section{Time Frequency Representation of Sound}
\label{sec:preliminaries}
\noindent Most machine learning models do not directly operate on the raw waveform i.e. a sequence  of air pressure measurements. Instead, it is first transformed from the time domain to the frequency domain exploiting the fact that arbitrarily complex waves can be represented as a combinations of simple sinusoids. The set of sinusoids that, when summed together, yields the signal  is called the spectrum.\\
In practice, the spectrum is computed using the Discrete Fourier Transform (DFT).
\begin{align}
    \label{eq:dft}
    \mathrm{DFT}[k] &= \sum_{n=0}^{T-1} \mathrm{x}[t] \cdot (\cos(\varphi) - i\sin(\varphi))\\
     \varphi &= k \frac{t}{T} 2\pi
\end{align}
The output of the DFT is a list of $T$ complex numbers $c_k = a_k +b_ki$ that are used to describe $T$ sinusoids with frequencies from $0$ to $T-1$. Therefore, the frequency resolution, the number of frequencies between $\mathrm{DFT}[k]$ and $\mathrm{DFT}[k+1]$, is given by $\frac{sr}{T}$ where $sr$ is the sampling rate of the signal. Moreover, the frequency of the $k$th bin is $k * (\frac{sr}{T})$.
For each $k$, $\mathrm{DFT}[k]$ correlates the signal with sine and cosine waveforms with increasing frequencies (waveform parameters $\varphi$ depend on $k$) using the dot product. This can be interpreted as measuring the presence of the waveforms in the signal. Both sine and cosine are needed to account for arbitrary phase shifts.
The correlation measurements for the sine and cosine waveforms are stored in the real and imaginary part of $c_k$, respectively. It is also common to use Eulers Formula to shorten (\ref{eq:dft}) by using:
\begin{equation}
    cos(\varphi) - sin(\varphi)i = e^{-\varphi\mathrm{i}}
\end{equation}
One can compute the magnitude $\vert c_k \vert$ and the phase of the $k$th frequency bin by $\sqrt{a_k^2+b_k^2}$ and $tanh^{-1}(\frac{b_k}{a_k})$, respectively. The magnitude then mesaures the strength of the presence of the $k$th frequency bin in the signal.\\
When attempting to include sinusiods above the Nyquist Limit $\frac{sr}{2}$, aliasing effects occur as these frequencies are undersampled  Therefore, one only considers frequencies up to the Nyquist Limit.\\
Applying the DFT on a complex, non-stationary signal, i.e. signals whose frequency characteristics change over time (e.g. a song) would result in a histogram like representation, coined periodogram, that neglects the temporal evolution of the signal. To alleviate this problem, one uses the Short-Time-Fourier Transformation (STFT). The STFT computes the DFT on small overlapping chunks of the signal using a windowing function, resulting in a sequence of periodograms that describes the presence and absence of the frequency components over time. In this case the maximum value of $k$ is not determined by $T$ but rather set to $\frac{sr}{2}$ since the number of samples in the window is too small to cover all possible frequencies. Note that this causes a trade-off between the temporal resolution and the frequency resolution.\\
The output is a matrix $S \in \mathbb{R}^{F \times T}$ with $F$ frequency bins and $T$ time frames and is called the spectrogram. Each cell represent the amplitude (the normalized squared magnitude) of the corresponding frequencies in that band.\\
To account for the fact that the human perception of pitch is logarithmic in nature, i.e. humans are more discriminative at lower frequencies and less discriminative at higher frequencies, one additionally transforms the frequency bins into the Mel-scale using the Mel-filterbank that is composed of overlapping triangular filters. The Mel-scale is an empirically defined perceptual scale that mirrors human perception. Filters are small for low frequencies and are of increasing width for higher frequencies. They aggregate the energy of consecutive frequency bins to describe how much energy exists in various frequency regions.
This can be seen as a re-binning procedure that alters the number of bins from $F$ to $\hat{F}$, $T < \hat{T}$ where $\hat{T}$ is the number of Mel-filtes used. Finally the log of the energies is taken to convert from amplitude to decibel (dB).
The resulting Mel-spectrogram is a compact visual representation of audio that can be used as input to a machine-learning pipeline. Moreover, the Mel-spectrogram can be treated as an image of the underlying signal and one can therefore resort to computer vision approaches such as convolutional neural networks (CNNs). 
% \section{\uppercase{Preliminaries}}
%In this section we briefly review the necessary preliminaries and formalize the ASD problem.

